First observation of the $\overline{B}_{s}^{0}\to\Lambda_{c}^{+}\overline{\Lambda}_{c}{}^{-}$ decay and evidence for the $\overline{B}^{0}\to\Lambda_{c}^{+}\overline{\Lambda}_{c}{}^{-}$ decay

A search is presented for the two-body charmed baryonic decays $\overline{B}_{(s)}^{0}\to\Lambda_{c}^{+}\overline{\Lambda}_{c}{}^{-}$, using a data sample collected by the LHCb experiment during 2011--2012 and 2015--2018 corresponding to an integrated luminosity of $9\,\mathrm{fb}^{-1}$. The first observation of the $\overline{B}_{s}^{0}\to\Lambda_{c}^{+}\overline{\Lambda}_{c}{}^{-}$ decay is reported with $6.2\sigma$ significance, along with $4.3\sigma$ evidence for the $\overline{B}^{0}\to\Lambda_{c}^{+}\overline{\Lambda}_{c}{}^{-}$ decay. The branching fractions are measured to be $\mathcal{B}{}(\overline{B}^{0}\to\Lambda_{c}^{+}\overline{\Lambda}_{c}{}^{-}) = (1.01^{+0.27}_{-0.28} \pm 0.08 \pm 0.15) \times 10^{-5}$ and $\mathcal{B}{}(\overline{B}_{s}^{0}\to\Lambda_{c}^{+}\overline{\Lambda}_{c}{}^{-}) = (5.0 \pm 1.3 \pm 0.5 \pm 0.8) \times 10^{-5}$, where the first uncertainty is statistical, the second systematic, and the third due to external inputs. These results provide novel experimental inputs for the theoretical framework describing two-body baryonic decays of $B$ mesons via $W$-emission and $W$-exchange mechanisms.

==> Authorship_LHCb-PAPER-2025-053-arXiv.tex <==
LHCb collaboration:
R. Aaij,
A.S.W. Abdelmotteleb,
C. Abellan Beteta,
F. Abudin{\'e}n,
T. Ackernley,
A. A.  Adefisoye,
B. Adeva,
M. Adinolfi,
P. Adlarson,
C. Agapopoulou,
C.A. Aidala,
Z. Ajaltouni,
S. Akar,
K. Akiba,
M.  Akthar,
P. Albicocco,
J. Albrecht,
R.  Aleksiejunas,
F. Alessio,
P. Alvarez Cartelle,
R. Amalric,
S. Amato,
J.L. Amey,
Y. Amhis,
L. An,
L. Anderlini,
M. Andersson,
P. Andreola,
M. Andreotti,
S.  Andres Estrada,
A. Anelli,
D. Ao,
C. Arata,
F. Archilli,
Z. Areg,
M. Argenton,
S. Arguedas Cuendis,
L.  Arnone,
A. Artamonov,
M. Artuso,
E. Aslanides,
R. Ata\'{i}de Da Silva,
M. Atzeni,
B. Audurier,
J. A.  Authier,
D. Bacher,
I. Bachiller Perea,
S. Bachmann,
M. Bachmayer,
J.J. Back,
P. Baladron Rodriguez,
V. Balagura,
A.  Balboni,
W. Baldini,
Z. Baldwin,
L. Balzani,
H.  Bao,
J. Baptista de Souza Leite,
C. Barbero Pretel,
M. Barbetti,
I. R. Barbosa,
R.J. Barlow,
M. Barnyakov,
S. Barsuk,
W. Barter,
J. Bartz,
S. Bashir,
B. Batsukh,
P. B.  Battista,
A.  Bavarchee,
A. Bay,
A. Beck,
M. Becker,
F. Bedeschi,
I.B. Bediaga,
N. A.  Behling,
S. Belin,
A.  Bellavista,
K. Belous,
I. Belov,
I. Belyaev,
G. Benane,
G. Bencivenni,
E. Ben-Haim,
A. Berezhnoy,
R. Bernet,
S. Bernet Andres,
A. Bertolin,
F. Betti,
J.  Bex,
O. Bezshyyko,
S.  Bhattacharya,
M.S. Bieker,
N.V. Biesuz,
A. Biolchini,
M. Birch,
F.C.R. Bishop,
A. Bitadze,
A. Bizzeti,
T. Blake,
F. Blanc,
J.E. Blank,
S. Blusk,
V. Bocharnikov,
J.A. Boelhauve,
O. Boente Garcia,
T. Boettcher,
A.  Bohare,
A. Boldyrev,
C. Bolognani,
R. Bolzonella,
R. B.  Bonacci,
N. Bondar,
A. Bordelius,
F. Borgato,
S. Borghi,
M. Borsato,
J.T. Borsuk,
E.  Bottalico,
S.A. Bouchiba,
M.  Bovill,
T.J.V. Bowcock,
A. Boyer,
C. Bozzi,
J. D. Brandenburg,
A. Brea Rodriguez,
N. Breer,
J. Brodzicka,
J. Brown,
D. Brundu,
E. Buchanan,
M.  Burgos Marcos,
A.T. Burke,
C. Burr,
C.  Buti,
J.S. Butter,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
Y.  Cai,
A. Caillet,
R. Calabrese,
S. Calderon Ramirez,
L. Calefice,
M. Calvi,
M. Calvo Gomez,
P. Camargo Magalhaes,
J. I. Cambon Bouzas,
P. Campana,
A. C. Campos,
A.F. Campoverde Quezada,
S. Capelli,
M.  Caporale,
L. Capriotti,
R. Caravaca-Mora,
A. Carbone,
L. Carcedo Salgado,
R. Cardinale,
A. Cardini,
P. Carniti,
L. Carus,
A. Casais Vidal,
R. Caspary,
G. Casse,
M. Cattaneo,
G. Cavallero,
V. Cavallini,
S. Celani,
I.  Celestino,
S.  Cesare,
A.J. Chadwick,
I. Chahrour,
H.  Chang,
M. Charles,
Ph. Charpentier,
E.  Chatzianagnostou,
R.  Cheaib,
M. Chefdeville,
C. Chen,
J.  Chen,
S. Chen,
Z. Chen,
A.  Chen Hu,
M.  Cherif,
A. Chernov,
S. Chernyshenko,
X.  Chiotopoulos,
V. Chobanova,
M. Chrzaszcz,
A. Chubykin,
V. Chulikov,
P. Ciambrone,
X. Cid Vidal,
G. Ciezarek,
P. Cifra,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
C. Cocha Toapaxi,
V. Coco,
J. Cogan,
E. Cogneras,
L. Cojocariu,
S.  Collaviti,
P. Collins,
T. Colombo,
M. Colonna,
A. Comerma-Montells,
L. Congedo,
J.  Connaughton,
A. Contu,
N. Cooke,
G. Cordova,
C.  Coronel,
I. Corredoira ,
A. Correia,
G. Corti,
J. Cottee Meldrum,
B. Couturier,
D.C. Craik,
M. Cruz Torres,
M.  Cubero Campos,
E. Curras Rivera,
R. Currie,
C.L. Da Silva,
S. Dadabaev,
L. Dai,
X. Dai,
E. Dall'Occo,
J. Dalseno,
C. D'Ambrosio,
J. Daniel,
G. Darze,
A.  Davidson,
J.E. Davies,
O. De Aguiar Francisco,
C. De Angelis,
F. De Benedetti,
J. de Boer,
K. De Bruyn,
S. De Capua,
M. De Cian,
U. De Freitas Carneiro Da Graca,
E. De Lucia,
J.M. De Miranda,
L. De Paula,
M. De Serio,
P. De Simone,
F. De Vellis,
J.A. de Vries,
F. Debernardis,
D. Decamp,
S.  Dekkers,
L. Del Buono,
B. Delaney,
J. Deng,
V. Denysenko,
O. Deschamps,
F. Dettori,
B. Dey,
P. Di Nezza,
I. Diachkov,
S. Didenko,
S. Ding,
Y.  Ding,
L. Dittmann,
V. Dobishuk,
A. D.  Docheva,
A.  Doheny,
C. Dong,
A.M. Donohoe,
F. Dordei,
A.C. dos Reis,
A. D.  Dowling,
L. Dreyfus,
W. Duan,
P. Duda,
L. Dufour,
V. Duk,
P. Durante,
M. M. Duras,
J.M. Durham,
O. D.  Durmus,
A. Dziurda,
A. Dzyuba,
S. Easo,
E. Eckstein,
U. Egede,
A. Egorychev,
V. Egorychev,
S. Eisenhardt,
E. Ejopu,
L. Eklund,
M. Elashri,
D.  Elizondo Blanco,
J. Ellbracht,
S. Ely,
A. Ene,
J. Eschle,
T. Evans,
F. Fabiano,
S.  Faghih,
L.N. Falcao,
B. Fang,
R. Fantechi,
L. Fantini,
M. Faria,
K.   Farmer,
F.  Fassin,
D. Fazzini,
L. Felkowski,
M. Feng,
A. Fernandez Casani,
M. Fernandez Gomez,
A.D. Fernez,
F. Ferrari,
F. Ferreira Rodrigues,
M. Ferrillo,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiorini,
M. Firlej,
K.L. Fischer,
D.S. Fitzgerald,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
A.  Fomin,
M. Fontana,
L. A.  Foreman,
R. Forty,
D. Foulds-Holt,
V. Franco Lima,
M. Franco Sevilla,
M. Frank,
E. Franzoso,
G. Frau,
C. Frei,
D.A. Friday,
J. Fu,
Q. F{\"u}hring,
T. Fulghesu,
G. Galati,
M.D. Galati,
A. Gallas Torreira,
D. Galli,
S. Gambetta,
M. Gandelman,
P. Gandini,
B.  Ganie,
H. Gao,
R. Gao,
T.Q. Gao,
Y. Gao,
Y. Gao,
Y. Gao,
L.M. Garcia Martin,
P. Garcia Moreno,
J. Garc{\'\i}a Pardi{\~n}as,
P.  Gardner,
L. Garrido,
C. Gaspar,
A.  Gavrikov,
L.L. Gerken,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
S. Ghizzo,
Z. Ghorbanimoghaddam,
F. I. Giasemis,
V. Gibson,
H.K. Giemza,
A.L. Gilman,
M. Giovannetti,
A. Giovent{\`u},
L. Girardey,
M.A. Giza,
F.C. Glaser,
V.V. Gligorov,
C. G{\"o}bel,
L.  Golinka-Bezshyyko,
E. Golobardes,
D. Golubkov,
A. Golutvin,
S. Gomez Fernandez,
W.  Gomulka,
I. Gonçales Vaz,
F. Goncalves Abrantes,
M. Goncerz,
G. Gong,
J. A. Gooding,
I.V. Gorelov,
C. Gotti,
E. Govorkova,
J.P. Grabowski,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
L. Grazette,
G. Graziani,
A. T. Grecu,
N.A. Grieser,
L. Grillo,
S. Gromov,
C.  Gu,
M. Guarise,
L.  Guerry,
A.-K. Guseinov,
E. Gushchin,
Y. Guz,
T. Gys,
K. Habermann,
T. Hadavizadeh,
C. Hadjivasiliou,
G. Haefeli,
C. Haen,
S.  Haken,
G.  Hallett,
P.M. Hamilton,
J. Hammerich,
Q. Han,
X. Han,
S. Hansmann-Menzemer,
L. Hao,
N. Harnew,
T. H.  Harris,
M. Hartmann,
S. Hashmi,
J. He,
N.  Heatley,
A.  Hedes,
F. Hemmer,
C. Henderson,
R. Henderson,
R.D.L. Henderson,
A.M. Hennequin,
K. Hennessy,
L. Henry,
J. Herd,
P. Herrero Gascon,
J. Heuel,
A.  Heyn,
A. Hicheur,
G. Hijano Mendizabal,
J. Horswill,
R. Hou,
Y. Hou,
D.C. Houston,
N. Howarth,
W. Hu,
X. Hu,
W. Hulsbergen,
R.J. Hunter,
M. Hushchyn,
D. Hutchcroft,
M. Idzik,
D. Ilin,
P. Ilten,
A. Iniukhin,
A.  Iohner,
A. Ishteev,
K. Ivshin,
H. Jage,
S.J. Jaimes Elles,
S. Jakobsen,
T. Jakoubek,
E. Jans,
B.K. Jashal,
A. Jawahery,
C.  Jayaweera,
A.  Jelavic,
V. Jevtic,
Z.  Jia,
E. Jiang,
X. Jiang,
Y. Jiang,
Y. J.  Jiang,
E. Jimenez Moya,
N.  Jindal,
M. John,
A.  John Rubesh Rajan,
D. Johnson,
C.R. Jones,
S. Joshi,
B. Jost,
J.  Juan Castella,
N. Jurik,
I. Juszczak,
K.  Kalecinska,
D. Kaminaris,
S. Kandybei,
M.  Kane,
Y. Kang,
C. Kar,
M. Karacson,
A. Kauniskangas,
J.W. Kautz,
M.K. Kazanecki,
F. Keizer,
M. Kenzie,
T. Ketel,
B. Khanji,
A. Kharisova,
S. Kholodenko,
G. Khreich,
F.  Kiraz,
T. Kirn,
V.S. Kirsebom,
S. Klaver,
N. Kleijne,
A. Kleimenova,
D. K.  Klekots,
K. Klimaszewski,
M.R. Kmiec,
T.  Knospe,
R.  Kolb,
S. Koliiev,
L. Kolk,
A. Konoplyannikov,
P. Kopciewicz,
P. Koppenburg,
A.  Korchin,
I. Kostiuk,
O. Kot,
S. Kotriakhova,
E.  Kowalczyk,
A. Kozachuk,
P. Kravchenko,
L. Kravchuk,
O.  Kravcov,
M. Kreps,
P. Krokovny,
W. Krupa,
W. Krzemien,
O. Kshyvanskyi,
S. Kubis,
M. Kucharczyk,
V. Kudryavtsev,
E. Kulikova,
A. Kupsc,
V. Kushnir,
B. Kutsenko,
J. Kvapil,
I.  Kyryllin,
D. Lacarrere,
P.  Laguarta Gonzalez,
A. Lai,
Y. Lai,
A. Lampis,
D. Lancierini,
C. Landesa Gomez,
J.J. Lane,
G. Lanfranchi,
C. Langenbruch,
J. Langer,
T. Latham,
F. Lazzari,
C. Lazzeroni,
R. Le Gac,
H.  Lee,
R. Lef{\`e}vre,
A. Leflat,
S. Legotin,
M. Lehuraux,
E. Lemos Cid,
O. Leroy,
T. Lesiak,
E. D. Lesser,
B. Leverington,
A. Li,
C.  Li,
C.  Li,
H. Li,
J. Li,
K. Li,
L. Li,
M. Li,
P. Li,
P.-R. Li,
Q.  Li,
T. Li,
T. Li,
Y. Li,
Y. Li,
Y.  Li,
Z. Lian,
Q.  Liang,
X. Liang,
Z.  Liang,
S. Libralon,
A.  Lightbody,
C. Lin,
T. Lin,
R. Lindner,
H.  Linton,
R. Litvinov,
D. Liu,
F. L.  Liu,
G. Liu,
K. Liu,
S. Liu,
W.  Liu,
Y. Liu,
Y. Liu,
Y. L.  Liu,
G. Loachamin Ordonez,
I.  Lobo,
A. Lobo Salvia,
A. Loi,
T. Long,
F. C. L. Lopes,
J.H. Lopes,
A. Lopez Huertas,
C.  Lopez Iribarnegaray,
S. L{\'o}pez Soli{\~n}o,
Q. Lu,
C. Lucarelli,
D. Lucchesi,
M. Lucio Martinez,
Y. Luo,
A. Lupato,
E. Luppi,
K. Lynch,
X.-R. Lyu,
G. M.  Ma,
H.  Ma,
S. Maccolini,
F. Machefert,
F. Maciuc,
B.  Mack,
I. Mackay,
L. M.  Mackey,
L.R. Madhan Mohan,
M. J.  Madurai,
D. Magdalinski,
D. Maisuzenko,
J.J. Malczewski,
S. Malde,
L. Malentacca,
A. Malinin,
T. Maltsev,
G. Manca,
G. Mancinelli,
C. Mancuso,
R. Manera Escalero,
F. M.  Manganella,
D. Manuzzi,
D. Marangotto,
J.F. Marchand,
R. Marchevski,
U. Marconi,
E. Mariani,
S. Mariani,
C. Marin Benito,
J. Marks,
A.M. Marshall,
L.  Martel,
G. Martelli,
G. Martellotti,
L. Martinazzoli,
M. Martinelli,
D.  Martinez Gomez,
D. Martinez Santos,
F. Martinez Vidal,
A.  Martorell i Granollers,
A. Massafferri,
R. Matev,
A. Mathad,
V. Matiunin,
C. Matteuzzi,
K.R. Mattioli,
A. Mauri,
E. Maurice,
J. Mauricio,
P. Mayencourt,
J. Mazorra de Cos,
M. Mazurek,
D.  Mazzanti Tarancon,
M. McCann,
N.T. McHugh,
A. McNab,
R. McNulty,
B. Meadows,
D. Melnychuk,
D. Mendoza Granada,
P.  Menendez Valdes Perez,
F. M.  Meng,
M. Merk,
A. Merli,
L. Meyer Garcia,
D. Miao,
H. Miao,
M. Mikhasenko,
D.A. Milanes,
A. Minotti,
E. Minucci,
T. Miralles,
B. Mitreska,
D.S. Mitzel,
R.  Mocanu,
A. Modak,
L. Moeser,
R.D. Moise,
E. F. Molina Cardenas,
T. Momb{\"a}cher,
M. Monk,
T. Monnard,
S. Monteil,
A. Morcillo Gomez,
G. Morello,
M.J. Morello,
M.P. Morgenthaler,
A.  Moro,
J. Moron,
W.  Morren,
A.B. Morris,
A.G. Morris,
R. Mountain,
Z. M.  Mu,
E. Muhammad,
F. Muheim,
M. Mulder,
K. M{\"u}ller,
F. Mu{\~n}oz-Rojas,
R. Murta,
V.  Mytrochenko,
P. Naik,
T. Nakada,
R. Nandakumar,
T. Nanut,
G.  Napoletano,
I. Nasteva,
M. Needham,
E.  Nekrasova,
N. Neri,
S. Neubert,
N. Neufeld,
P. Neustroev,
J. Nicolini,
D. Nicotra,
E.M. Niel,
N. Nikitin,
L.  Nisi,
Q. Niu,
B. K. Njoki,
P. Nogarolli,
P. Nogga,
C. Normand,
J. Novoa Fernandez,
G. Nowak,
C. Nunez,
H. N.  Nur,
A. Oblakowska-Mucha,
V. Obraztsov,
T. Oeser,
A. Okhotnikov,
O. Okhrimenko,
R. Oldeman,
F. Oliva,
E.  Olivart Pino,
M. Olocco,
R.H. O'Neil,
J.S. Ordonez Soto,
D. Osthues,
J.M. Otalora Goicochea,
P. Owen,
A. Oyanguren,
O. Ozcelik,
F. Paciolla,
A.  Padee,
K.O. Padeken,
B. Pagare,
T. Pajero,
A. Palano,
L.  Palini,
M. Palutan,
C.  Pan,
X.  Pan,
S. Panebianco,
S. Paniskaki,
G. Panshin,
L. Paolucci,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
C. Pappenheimer,
C. Parkes,
D.  Parmar,
G. Passaleva,
D. Passaro,
A. Pastore,
M. Patel,
J. Patoc,
C. Patrignani,
A.  Paul,
C.J. Pawley,
A. Pellegrino,
J.  Peng,
X.  Peng,
M. Pepe Altarelli,
S. Perazzini,
D. Pereima,
H.  Pereira Da Costa,
M.  Pereira Martinez,
A. Pereiro Castro,
C.  Perez,
P. Perret,
A.  Perrevoort,
A. Perro,
M.J. Peters,
K. Petridis,
A. Petrolini,
S.  Pezzulo,
J. P.  Pfaller,
H. Pham,
L. Pica,
M. Piccini,
L.  Piccolo,
B. Pietrzyk,
G. Pietrzyk,
R. N. Pilato,
D. Pinci,
F. Pisani,
M. Pizzichemi,
V. M. Placinta,
M. Plo Casasus,
T. Poeschl,
F. Polci,
M. Poli Lener,
A. Poluektov,
N. Polukhina,
I. Polyakov,
E. Polycarpo,
S. Ponce,
D. Popov,
K. Popp,
S. Poslavskii,
K. Prasanth,
C. Prouve,
D. Provenzano,
V. Pugatch,
A.  Puicercus Gomez,
G. Punzi,
J.R. Pybus,
Q. Q.  Qian,
W. Qian,
N. Qin,
R. Quagliani,
R.I. Rabadan Trejo,
R.  Racz,
J.H. Rademacker,
M. Rama,
M.  Ram\'{i}rez Garc\'{i}a,
V. Ramos De Oliveira,
M. Ramos Pernas,
M.S. Rangel,
F. Ratnikov,
G. Raven,
M. Rebollo De Miguel,
F. Redi,
J. Reich,
F. Reiss,
Z. Ren,
P.K. Resmi,
M.  Ribalda Galvez,
R. Ribatti,
G. Ricart,
D. Riccardi,
S. Ricciardi,
K. Richardson,
M. Richardson-Slipper,
F.  Riehn,
K. Rinnert,
P. Robbe,
G. Robertson,
E. Rodrigues,
A. Rodriguez Alvarez,
E. Rodriguez Fernandez,
J.A. Rodriguez Lopez,
E. Rodriguez Rodriguez,
J. Roensch,
A. Rogachev,
A. Rogovskiy,
D.L. Rolf,
P. Roloff,
V. Romanovskiy,
A. Romero Vidal,
G. Romolini,
F. Ronchetti,
T. Rong,
M. Rotondo,
S. R.  Roy,
M.S. Rudolph,
M. Ruiz Diaz,
R.A. Ruiz Fernandez,
J. Ruiz Vidal,
J. J. Saavedra-Arias,
J.J. Saborido Silva,
S. E. R. Sacha Emile R.,
N. Sagidova,
D. Sahoo,
N. Sahoo,
B. Saitta,
M. Salomoni,
I. Sanderswood,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
L. Santoro ,
E. Santovetti,
A. Saputi,
D. Saranin,
A. Sarnatskiy,
G. Sarpis,
M. Sarpis,
C. Satriano,
A. Satta,
M. Saur,
D. Savrina,
H. Sazak,
F. Sborzacchi,
A. Scarabotto,
S. Schael,
S. Scherl,
M. Schiller,
H. Schindler,
M. Schmelling,
B. Schmidt,
N. Schmidt,
S. Schmitt,
H. Schmitz,
O. Schneider,
A. Schopper,
N. Schulte,
M.H. Schune,
G. Schwering,
B. Sciascia,
A. Sciuccati,
G.  Scriven,
I. Segal,
S. Sellam,
A. Semennikov,
T. Senger,
M. Senghi Soares,
A. Sergi,
N. Serra,
L. Sestini,
A. Seuthe,
B.  Sevilla Sanjuan,
Y. Shang,
D.M. Shangase,
M. Shapkin,
R. S.  Sharma,
I. Shchemerov,
L. Shchutska,
T. Shears,
L. Shekhtman,
Z. Shen,
S. Sheng,
V. Shevchenko,
B. Shi,
J.  Shi,
Q. Shi,
W. S.  Shi,
Y. Shimizu,
E. Shmanin,
R. Shorkin,
J.D. Shupperd,
R. Silva Coutinho,
G. Simi,
S. Simone,
M.  Singha,
I. Siral,
N. Skidmore,
T. Skwarnicki,
M.W. Slater,
E. Smith,
M. Smith,
L. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
A. Solomin,
A. Solovev,
K.  Solovieva,
N. S.  Sommerfeld,
R. Song,
Y. Song,
Y. Song,
Y. S.  Song,
F.L. Souza De Almeida,
B. Souza De Paula,
K.M. Sowa,
E. Spadaro Norella,
E. Spedicato,
J.G. Speer,
P. Spradlin,
F. Stagni,
M. Stahl,
S. Stahl,
S. Stanislaus,
M.  Stefaniak,
O. Steinkamp,
D. Strekalina,
Y. Su,
F. Suljik,
J. Sun,
J.  Sun,
L. Sun,
D. Sundfeld,
W. Sutcliffe,
P. Svihra,
V. Svintozelskyi,
K. Swientek,
F. Swystun,
A. Szabelski,
T. Szumlak,
Y. Tan,
Y. Tang,
Y. T.  Tang,
M.D. Tat,
J. A. Teijeiro Jimenez,
A. Terentev,
F. Terzuoli,
F. Teubert,
E. Thomas,
D.J.D. Thompson,
A. R.  Thomson-Strong,
H. Tilquin,
V. Tisserand,
S. T'Jampens,
M. Tobin,
T. T.  Todorov,
L. Tomassetti,
G. Tonani,
X. Tong,
T. Tork,
L. Toscano,
D.Y. Tou,
C. Trippl,
G. Tuci,
N. Tuning,
L.H. Uecker,
A. Ukleja,
D.J. Unverzagt,
A.  Upadhyay,
B.  Urbach,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
V. Vagnoni,
A.  Vaitkevicius,
V.  Valcarce Cadenas,
G. Valenti,
N. Valls Canudas,
J. van Eldik,
H. Van Hecke,
E. van Herwijnen,
C.B. Van Hulse,
R. Van Laak,
M. van Veghel,
G. Vasquez,
R. Vazquez Gomez,
P. Vazquez Regueiro,
C. V{\'a}zquez Sierra,
S. Vecchi,
J.  Velilla Serna,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Verdoglia,
M. Vesterinen,
W. Vetens,
D.  Vico Benet,
P.  Vidrier Villalba,
M. Vieites Diaz,
X. Vilasis-Cardona,
E. Vilella Figueras,
A. Villa,
P. Vincent,
B. Vivacqua,
F.C. Volle,
D. vom Bruch,
N. Voropaev,
K. Vos,
C. Vrahas,
J. Wagner,
J. Walsh,
E.J. Walton,
G. Wan,
A.  Wang,
B.  Wang,
C. Wang,
G. Wang,
H. Wang,
J. Wang,
J. Wang,
J. Wang,
J. Wang,
L. Wang,
M. Wang,
N. W.  Wang,
R. Wang,
X. Wang,
X. Wang,
X. W.  Wang,
Y. Wang,
Y. Wang,
Y. H.  Wang,
Z. Wang,
Z. Wang,
J.A. Ward,
M. Waterlaat,
N.K. Watson,
D. Websdale,
Y. Wei,
Z.  Weida,
J. Wendel,
B.D.C. Westhenry,
C. White,
M. Whitehead,
E. Whiter,
A.R. Wiederhold,
D. Wiedner,
M. A. Wiegertjes,
C.  Wild,
G. Wilkinson,
M.K. Wilkinson,
M. Williams,
M. J. Williams,
M.R.J. Williams,
R. Williams,
S.  Williams,
Z.  Williams,
F.F. Wilson,
M. Winn,
W. Wislicki,
M. Witek,
L. Witola,
T. Wolf,
E.  Wood,
G. Wormser,
S.A. Wotton,
H. Wu,
J. Wu,
X. Wu,
Y. Wu,
Z. Wu,
K. Wyllie,
S. Xian,
Z. Xiang,
Y. Xie,
T. X.  Xing,
A. Xu,
L. Xu,
M. Xu,
Z. Xu,
Z. Xu,
Z. Xu,
S.  Yadav,
K.  Yang,
X. Yang,
Y. Yang,
Y.  Yang,
Z. Yang,
V. Yeroshenko,
H. Yeung,
H. Yin,
X.  Yin,
C. Y.  Yu,
J. Yu,
X. Yuan,
Y Yuan,
J. A. Zamora Saa,
M. Zavertyaev,
M. Zdybal,
F. Zenesini,
C.  Zeng,
M. Zeng,
C. Zhang,
D. Zhang,
J. Zhang,
L. Zhang,
R. Zhang,
S. Zhang,
S.~L.~  Zhang,
Y. Zhang,
Y. Z.  Zhang,
Z. Zhang,
Y. Zhao,
A. Zhelezov,
S. Z.  Zheng,
X. Z.  Zheng,
Y. Zheng,
T. Zhou,
X. Zhou,
Y. Zhou,
V. Zhovkovska,
L. Z.  Zhu,
X. Zhu,
X. Zhu,
Y.  Zhu,
V. Zhukov,
J. Zhuo,
D. Zuliani,
G. Zunica
